Morpheus: Safe and Flexible Dynamic Updates for SDNs

SDN controllers must be periodically modified to add features, improve performance, and fix bugs, but current techniques for implementing dynamic updates are inadequate. Simply halting old controllers and bringing up new ones can cause state to be lost, which often leads to incorrect behavior-e.g., if the state represents hosts blacklisted by a firewall, then traffic that should be blocked may be allowed to pass through. Techniques based on record and replay can reconstruct state automatically, but they are expensive to deploy and can lead to incorrect behavior. Problematic scenarios are especially likely to arise in distributed controllers and with semantics-altering updates. This paper presents a new approach to implementing dynamic controller updates based on explicit state transfer. Instead of attempting to infer state changes automatically-an approach that is expensive and fundamentally incomplete-our framework gives programmers effective tools for implementing correct updates that avoid major disruptions. We develop primitives that enable programmers to directly (and easily, in most cases) initialize the new controller's state as a function of old state and we design protocols that ensure consistent behavior during the transition. We also present a prototype implementation called Morpheus, and evaluate its effectiveness on representative case studies.

==> Makefile <==
TEX      := latex
PDFTEX   := pdflatex
BIBTEX   := bibtex
RM       := rm -f
OPTIONS  = -o
PDFTEXOPTIONS = --interaction batchmode

SRC     = paper
PAPER   = $(SRC).pdf

BIBSRC  = $(shell ls *.bib)
BIBFILE = $(shell ls *.bbl)

all: $(PAPER)

%.pdf: %.dvi 
	clear
	echo Running $(PDFTEX)
	$(PDFTEX) $(PDFTEXOPTIONS) $(basename $*);\

%.dvi: $(AUTOGEN_PDFS) $(shell ls *.tex) 
	clear
	echo Running $(PDFTEX)
	echo $(basename $@) 
	$(PDFTEX) $(basename $@)
	clear
	echo Running $(BIBTEX);\
	$(BIBTEX) $(basename $@) ;\
	clear;\
	for i in 1 2; do\
	   echo Running $(PDFTEX);\
	   $(PDFTEX) $(basename $@) ;\
	done

clean: 
	$(RM) $(PAPER) *.dvi *.bbl *.aux *.log *blg *~

